Aerostructural Wing Shape Optimization assisted by Algorithmic Differentiation

With more efficient structures, last trends in aeronautics have witnessed an increased flexibility of wings, calling for adequate design and optimization approaches. To correctly model the coupled physics, aerostructural optimization has progressively become more important, being nowadays performed also considering higher-fidelity discipline methods, i.e., CFD for aerodynamics and FEM for structures. In this paper a methodology for high-fidelity gradient-based aerostructural optimization of wings, including aerodynamic and structural nonlinearities, is presented. The main key feature of the method is its modularity: each discipline solver, independently employing algorithmic differentiation for the evaluation of adjoint-based sensitivities, is interfaced at high-level by means of a wrapper to both solve the aerostructural primal problem and evaluate exact discrete gradients of the coupled problem. The implemented capability, ad-hoc created to demonstrate the methodology, and freely available within the open-source SU2 multiphysics suite, is applied to perform aerostructural optimization of aeroelastic test cases based on the ONERA M6 and NASA CRM wings. Single-point optimizations, employing Euler or RANS flow models, are carried out to find wing optimal outer mold line in terms of aerodynamic efficiency. Results remark the importance of taking into account the aerostructural coupling when performing wing shape optimization.

==> Chapters/2_Introduction.tex <==
%------------------------------------------%
\section{Introduction}
\label{sec:intro}
%------------------------------------------%
%
\inred{seconda passata Rocco}\newline
Multi-Disciplinary Optimization (MDO) applied to aircraft design has been attracting the interest of both research and industry for the last fifty years~\cite{QualcosadiMartin}. 
Currently it's a widely researched topic, as witnessed by recent EU funded projects~\cite{AGILE,AGILE4.0}. 
%
Anyway, regardless of the advancements, MDO is still not  applicable to reproduce, with high level of confidence, the complex interaction of the disciplines within the context of aircraft design. 
Due to this, several different philosophies are typically found in the literature. A common one, which also fits well the needs of early aircraft design stages, is to model the different disciplines with low-fidelity physics~\cite{Kennedy2014e,Chauhan2018LowFidelityAO,Jasa2018OpensourceCA,Elham2015}. On the other side of the spectrum, the driving idea is to reduce the number of concurrently considered disciplines and model each of them with high-fidelity physics: this last option is more suitable for later design phases. 
%%
\par
%Aerostructural
Two of the most relevant disciplines driving an aircraft design are aerodynamics and structures. 
Their interaction concurs in causing a wide range of aeroelastic phenomena. 
Typically, aerostructural optimization considers as  state (or discipline) equations the ones relative to the steady aerodynamics and solid mechanics. Common Design Variables (DVs) consist in aerodynamic shapes and/or structural parameters (e.g., thickness of the skin), while constraints consider the integrity of the structure and/or the trim of the aircraft (mainly in terms of lift to be generated). Very often, constraints and/or objective function regard aircraft performances, such as, range, which in turn, depends on aircraft weight and aerodynamic efficiency.
%
A fundamental aspect may be the coupling between the physics of the two considered discipline: for a given flight condition, the deflect shape of the wing is tightly coupled with aerodynamic forces in a two-way relation. 
With the current trends to design structurally efficient structures, the deformed wing shape in flight conditions are remarkable, exacerbating the need for including such coupling into the optimization.
Different optimization strategies in which other aeroelastic phenomena are included have also been carried out (e.g., considering flutter speed), however, efforts featuring mainly aerostructural optimization problems will be reviewed in the following.  
%
\par
%
% Haftka
Efforts in the aerostructural optimization were initiated by Haftka~\cite{HAFTKA-1977} who proposed a method for the optimization of flexible wings subjected to stress, strain  and drag constraints. The adopted fidelity level of the discipline tools reflected the availability of that times, and consisted in a Lifting Line Method (LLM) for aerodynamics and a Finite Element Method (FEM) for the structure. 
A penalty method formulation was converting the constrained problem into an unconstrained one. 
% Grossman
Later on, Grossman \textit{et al.}~\cite{GROSSMAN_1986} applied an integrated aircraft design analysis and optimization on a sailplane, employing a LLM and  beam-based FEM. 
They explored two optimization strategies: in the first one, aerodynamics and structure where optimized sequentially, i.e. isolated aerodynamic and structural optimizations were repeatedly performed,  while in the second, an integrated (concurrent) procedure was used. 
They showed how the integrated approach is superior to the iterative approach, capitalizing on the interaction between disciplines and finding better results with respect to sub-optimal ones, given by sequential optimization. A physical interpretation of the different outcomes was also provided.
%
%Grossman 2
Following this last work, a higher-fidelity aerostructural model was later used for the optimization of the weight of a forward-swept subsonic aircraft wing subjected to range constraint~\cite{GROSSMAN_1989}. 
%For the aerodynamics, a vortex lattice method was used and viscous drag estimation was computed using section lift coefficient and drag polar, based on provided data; various design variables were employed, based on geometry, structure and performance requirements. 
%
Regarding the performances of sequential/integrated approaches, recently Martins~\textit{et al.}\cite{Martins2004HighFidelityAD} confirmed the observed trends also with higher-fidelity approaches.
%The advantage of coupled aerostructural optimization with respect to the sequential one was also recently confirmed by Martins \textit{et al.}\cite{Martins2004HighFidelityAD} employing an Euler flow model within the context of their aerostructural solver.
%
\par
%
In the last twenty years, researchers have started to employ higher-fidelity tools to perform aerostructural optimization. 
Such increased level of fidelity came with several consequences, being the first one an increased computational demand for each of the disciplines. When considering CFD, a further consequence is the need to consider a volume mesh that deforms when wing shape changes, both as consequence of the design change and the deflection in exercise. A high-level physics modeling (i.e. transonic aerodynamics~\cite{UC3M_ASO1Pustina}) generally requires an increased number of DVs to fully exploit the potentials of the optimization process. 
For such driving reasons, gradient-based optimization is generally preferred~\cite{qualcosaadjoint}, as it converges faster to a minimum; even though often-local, due to the non-convexity of the problem.
%As further measure to increase efficiency, adjoint methods to evaluate the sensitivity is adopted as it is not time-intensive (although depending on the strategy, large memory peaks can be reached).
%
\par
%  Maute
One of the pioneering works in this direction is the one of Maute \textit{et al.}~\cite{maute_2001}, featuring a gradient-based optimization framework with a three-field approach (structures, aerodynamics, mesh) to model the the nonlinear coupled problem. 
A staggered (also known as partitioned or segregated) procedure was set up to solve the coupled fields; aerodynamics was modeled with CFD-Euler, structure with a linear FE model and fluid mesh deformation with a spring-analogy method. 
Among the various proposed application the drag over lift ratio of the ARW2 wing was optimized, employing lift stress and displacement constraints while using as DVs backsweep angle, twist and structure thicknesses.
%, employing a staggered procedure for the solution (also known as partitioned or segregated). Aerodynamics consisted in an Euler flow model, structure in a linear FEM model and the motion of the fluid grid was computed by means of a spring analogy method. 
For the evaluation of sensitivity a direct approach was chosen, in which partial derivatives where analytically calculated and a staggered scheme was used to solve the system of equations. Direct approach is, anyway, only advantageous when then number of design variables is contained.
The authors stated that three-field formulations are on average 25\% slower than two-field ones (i.e. strategies that bypass fluid mesh deformation problem) but allow for bigger displacements in the structure, making it more general and reliable for a variety of cases. 
%
\par
%%%  Martins 1 & 2
Martins \textit{et al.}~\cite{martins2001ab} proposed a framework for the calculation of coupled aerostructural sensitivities for cases in which aeroelastic interactions were significant. 
The method employed high-fidelity models for both aerodynamics (CFD-Euler) and structure (linear FEM with two element types).  
%
This work is considered, to the best of the authors' knowledge, one of the first efforts to employ an adjoint method for the evaluation of aerostructural sensitivities~\cite{Martins_Review_Der2013} which makes the sensitivities evaluation time almost non-dependent of the number of the chosen DV (although, depending on the implementation, large memory peaks can be reached). 
%
\inred{[X RAUNO:Occhio da controllare se non fosse gia' stato usato su low fidelity, ci sono papers negli anni 90 che controllero']}.
%Such method allows a faster evaluation of sensitivities in case of a high number of design variables, making the computational time and cost to be almost independent of their number and, for such reason, the ideal to be applied for industrial cases. 
The proposed sensitivity evaluation framework is a lagged-coupled adjoint, in which the single discipline adjoint equations are lagged in a similar fashion of the primal solver solution strategy, and partial derivatives are evaluated analytically or by finite differences (FD). The proposed implementation was able to calculate aerostructural sensitivity of drag coefficient $C_D$ with respect to bump shape functions applied to the wing jig-shape. 
Their accuracy was compared both to FD and complex step (CP)-based sensitivities.
%
%
\par
%
%%%%% Martins 2004
Later on \cite{Martins2004HighFidelityAD} a similar framework was applied to the design of a supersonic business jet, pursuing the optimization of an objective function mixing weight and drag coefficient evaluated for a design lift coefficient; Kreisselmeier-Steinhauser function to lump individual stresses of the structure. A total number of 97 design variables was used representing both structural and aerodynamic shapes. Gradient evaluation time was observed to be almost independent of the number of DVs.
%
\par
%
%%%%  BARCELOS
Following their previous effort~\cite{maute_2001}, Maute \textit{et al.}~\cite{maute2003911} proposed a different method for aeroelastic optimization. For the same aerostructural problem, gradient calculation was achieved by analytically deriving the adjoint-based sensitivity equations of the primal problem: a staggered solution algorithm was implemented, where partial derivatives could be calculated analytically or by automatic differentiation. They also pointed out the computational problems relative to store partial derivative matrices of large-scale problems for adjoint-based sensitivity calculations. 
%
%\par
%
%In a following effort\cite{Martins2004HighFidelityAD}, Martins \textit{et al.} used a similar optimization framework  to optimize the design of a supersonic business jet. In this framework the flow was modeled with Euler equations while the structure consisted in a detailed linear FEM model. A comparison of adjoint-based sensitivities with FD and CP-based ones showed an average error of 2\%. The optimization was performed minimizing a combination of the aircraft $C_D$  and weight, constraining its $C_L$ and the Kreisselmeier-Steinhauser function to lump individual stresses of the structure. A total number of 97 design variables was used, divided into structural and aerodynamic surface ones, showing the almost independence of the gradient evaluation time from their number.
%
\par
%%%%  BARCELOS 
The work of Barcelos \textit{et al.}~\cite{Barcelos20081813} presented an optimization methodology for fluid-structure interaction (FSI) problems in which aerodynamic evaluation was based on turbulent flow models, namely RANS with Spalart-Allmaras (SA) turbulence model~\cite{SpallartAllmaraspaper}. 
The method employed the  three-field formulation strategy used in Maute \textit{et al.}~\cite{maute_2001,maute2003911}, while the structure was modeled via a geometrically nonlinear FEM. 
This counts, to the best of the authors' knowledge, as the highest level of fidelity adopted so far for aerostructural optimization of wings. 
Calculation of sensitivities followed the direct approach; all partial derivatives contribution were evaluated analytically or via FD. 
With the direct approach, evaluation of total derivatives of the state variables for the coupled aerostructural problem needs to be repeated for each design variable.
Nevertheless it was considered an advantageous approach compared to the adjoint one in case of large-scale problems, for which the Jacobian of the flow problem is difficult to transpose and keep in memory to be used at need.
%; nevertheless, the authors preferred this approach to the adjoint one to overcome issues related to storage of the Jacobian of the flow problem.
%in case of large-scale problems, for which the Jacobian of the flow problem is difficult to transpose and keep in memory to be used at need. 
\inblue{This is one of the common drawbacks due to memory requirements when using adjoint-based sensitivity evaluation strategies, largely mentioned in literature~\cite{maute2003911,SanchezThesis} which, in \inred{our} effort, is conveniently solved with the use of the library CoDiPack~\cite{sagebaum2017high} for Algorithmic Differentiation (AD).}
%
\par
%
%%% Brezillon
Other efforts presented gradient-based aerostructural optimizations using adjoint methods. Brezillion \textit{et al.}~\cite{Brezillon2012} proposed an articulated high-fidelity optimization framework wrapping DLR's TAU code for CFD (RANS-SA) which includes a discrete-adjoint model with non-frozen turbulence and ANSYS for linear structural FEM. 
%It is claimed, here, that relying only on high-fidelity models, besides being very costly, is unnecessary, and that multi-fidelity optimization strategies should be considered.
%
\par
%%% Ghazlane 
A similar approach was pursued by Ghazlane \textit{et al.}~\cite{ghazlane2012}. 
In the presented aerostructural framework, aerodynamics (with Euler flow model) was simulated by ONERA's \empj{elsA} code~\cite{Cambier2002}, which used an iterative fixed-point scheme for the solution of the aerodynamic adjoint; for the structure, a linear structural FEM module was analytically differentiated. 
%\inred{[Si, ma il coupling come?]}
%
\par
%%% Kenway 1 e 2
In effort~\cite{kenway2014} Kenway \textit{et al.} introduced a high-fidelity framework that could perform aerostructural optimization with respect to thousands of multidisciplinary variables, thanks to an improved parallel scalability of the method; a fully-coupled Newton-Krylov approach was employed for the solution of the aerostructural and the relative adjoint systems.  %%%%%%%%%
The aerostructural solver was based, for the aerodynamic part,  on SUmb~\cite{Weide2006} code, featuring  automatic differentiation (ADjoint), and, for the structural part, on TACS\cite{TACS2010}, also able to evaluate adjoint-based sensitivities. 
In the cited effort Euler flow model was used together with a linear detailed FEM model of the structure. 
To solve the aerostructural adjoint equations a combination of analytic, forward, and reverse AD methods was adopted.
The method was demonstrated on an aerostructural CRM test case~\cite{Vassberg-2008} using a CFD mesh with over than $16$~millions cells, a FEM grid with over 1 million degrees of freedom (DOFs) and more than $8$~millions state variables, using 512 processors. 
One of the purposes of the use of such large number of DOFs and DVs was that, even though adjoint-based gradient evaluation techniques should be almost independent of the number of considered design variables, in all previous efforts in literature their number had been limited: this because the real scalability of the method can only be achieved with a careful parallelization of its implementation
%One of the purpose of such large nuber of DOFs and DVs was overcoming the state of art at the time, which didn't really investigate the practical independence of adjoint-based gradient evaluation techniques on the number of DVs: in fact, real scalability of the method can only be achieved with a careful parallelization of its implementation. 
Similarly, in another study~\cite{KenwayMultipoint2014} Kenway \textit{et al.} presented a multipoint high-fidelity aerostructutal optimization of a CRM aeroelastic model, alternatively minimizing the takeoff gross weight and the fuel burn. 
%The CRM detailed CSM is built based on its aerodynamic mold line at 1 \textit{g} load factor. 
Flow model was based on Euler equation with a low fidelity viscous drag estimate; linearly behaving structures were considered. A massive parallel supercomputer (more than 400 processors) performed the calculations. \inred{[Dare occhiata a Krylov vs Block Gauss]}.
%
\par
%% Kennedy
A similar work was carried on by Kennedy \textit{et al.}\cite{Kennedy2014e} optimizing a Quasi-CRM wing model introducing also composite materials for the structure. 
After an aero-structural optimization based on lower-fidelity tools, a final RANS-based (SUmb) aerodynamic shape optimization was performed over the winner configuration.
Further studies were conducted by the authors~\cite{kennedyScitech2014}, in which RANS-based aerostructural optimizations were performed on the same model.
%
%Gradient-based aerostructural optimization is carried out using medium-fidelity tools: a combination of a panel method enhanced with induced and viscous drag evaluation (Tripan) together with a linear structural model (TACS). For coupled aerostructural adjoint analytic derivatives are implemented in the framework. After an aerostructural optimization which aims at minimizing a linear combination of takeoff gross weight and fuel burn a final RANS-based (SUmb) aerodynamic shape optimization is performed over the winner configuration aiming at minimizing $C_D$. Add on to the study is done by the authors in a follwing effort~\cite{kennedyScitech2014}, in which RANS-based aerostructural optimizations are performed on the same aeroelastic model.
%
\par
%%%% Kennedy undeflected 
Works of Kenway \textit{et al.}~\cite{KenwayScitech2014} and Brooks \textit{et al.}~\cite{Brooks2018} performed a similar RANS-based aerostructural optimization on variations of the NASA CRM (undeflected and higher aspect ratio versions) using a similar computational infrastructure as the one mentioned above by the same authors.  
%
%are dedicated to define, with an inverse design procedure and for aerostructural optimization purposes, undeflected versions with different Aspect Ratios (AR) of the CRM (uCRM). This because the CRM is born as aerodynamic benchmark only and its outer mold line represents the aerodynamic shape for 1 \textit{g} load factor. 
For the found configurations gradient-based aerostructural optimizations were performed, employing RANS-based CFD and linear FEM model with a similar computational infrastructure as the one mentioned above by the same authors. 
%
\par
%%%%% Hoogervorst
The study of Hoogervorst \textit{et al.}\cite{Hoogervorst2017WingAO} proposed an unconventional approach in the landscape of gradient-based aerostructural optimization. The selected MDO architecture was based on an individual discipline feasible (IDF) approach: the disciplines of the aerostructural problem were decoupled and convergence was ensured imposing additional equality constraints on the interdisciplinary state variables, which became additional design surrogate variables. 
This ensured to keep low the computational cost of the problem, especially in cases of strong nonlinearities, but only when the increase in design variables was kept low. 
In the study, flow was modeled with the Euler equation using the open-source code SU2~\cite{SU2_AIAAJ2016} while the analysis tool FEMWET was used to solve the linear structural equations. A combination of continuous adjoint approach and FD was used for gradient evaluation. The method was applied to reduce the fuel weight of an Airbus A320 aircraft for the specified range. %
DVs were both relative to external shape and structural thicknesses, together with the additional surrogate variables requested by the approach.
%geometric shapes Design variables are defined as the displacements of a Free-Form Deformation (FFD) box control points and selected structural model panels thicknesses, together with the additional surrogate variables requested by the approach.
%
\par
%
Finally, an example of genetic-based aerostructural optimization algorithm was proposed by Nikbay \textit{et al.}~\cite{Nickbay2009} who opted for a more industry-oriented strategy, in which the commercial software \emph{modeFRONTIER} was used to wrap various commercial codes (FLUENT for Euler-based aerodynamics, ABAQUS for linear FEM-based structure and CATIA for parametric solid geometry handling) to perform a loosely coupled analysis. The framework was built to handle the interfaces between such codes and the approach was validated on two aeroelastic test cases: the AGARD 445.6 wing and the ARW-2 wing. The motivation of such effort is that corporate working cultures need to rely (partially or entirely) on assessed commercial codes and a winning strategy should be to provide modular optimization frameworks for which each unit (conveniently interfaced) can be plugged and used.
%%%%%%  LOW FIDELITY 
%Another conspicuous branch of works in the field of aerostructural optimization relies on the use of low-medium fidelity aerodynamic models for the aeroelastic system. This is justified by the fact that using only high fidelity models in MDO makes the problem computationally too expensive to be employed in early design stages, where multiple designs are being considered at the same time. Besides the already mentioned work of of Kennedy \textit{et al.}~\cite{Kennedy2014e}, it is worth reporting efforts of Chauhan \textit{et al.}~\cite{Chauhan2018LowFidelityAO} and Jasa \textit{et al.}~\cite{Jasa2018OpensourceCA}, employing OpenAeroStruct: an open-source aerostructural optimization framework which couples a Vortex Lattice Method (VLM) to a 1D FEM to model lifting surfaces and uses coupled adjoint for gradient-based optimization, performed by means of NASA's OpenMDAO~\cite{OpenMDAO2012}. The framework presented by Elham \textit{et al.}~\cite{Elham2015} is a method for aerostructural optimization based on a VLM for aerodynamics and a beam model for structural FEM. With the enhancement of a viscous compressible airfoil drag prediction code, it is claimed to have a level of accuracy comparable to higher fidelity CFD-based tools. Sensitivities are evaluated with a combination of coupled adjoint method, automatic differentiation and chain rule differentiation.
%
%%%%%%%%%%%%%%
\subsection{Contributions of the present study}
%%%%%%%%%%%%%%
\inred{Sono qui}.
The studies mentioned above represent, mostly in chronological order,  a part of the attempt of the aerospace community to perform high-fidelity, i.e., employing CFD for aerodynamics and FEM for structures, coupled aerostructural optimization of aircraft wings.
%, with particular emphasis on frameworks relying on high-fidelity CFD and CSM models. 
This effort falls into such high-fidelity aerostructural optimization class; however several relevant and original contributions are brought at different levels. 
%
\par
Main contribution of this work is to introduce an open-source, high-fidelity framework for aerostructural design and optimization of wings, including aerodynamic and structural nonlinearities. The proposed gradient-based optimization  relies on an innovative and, to the best of the author's knowledge, never used strategy, based on coupled AD for gradient evaluation, which includes nonlinearities both in the CFD and CSM problems. 


\emph{First}, the code is completely open-source


\emph{Second}
builds upon 


Main contribution of this work is to introduce an open-source, high-fidelity framework for aerostructural design and optimization of wings, including aerodynamic and structural nonlinearities. The proposed gradient-based optimiz  relies on an innovative and, to the best of the author's knowledge, never used strategy, based on coupled AD for gradient evaluation, which includes nonlinearities both in the CFD and CSM problems. 
The framework, to be part of the open-source SU2 suite~\cite{Palacios2015, Pini2017, Gori2017, Molina2017, Zhou2017, albring2016}, relies on SU2 for high-fidelity CFD (Euler, RANS) and on a geometrically nonlinear beam FEM solver, namely pyBeam. Differently than previous efforts, in which FSI optimization problems were tackled by SU2 at native level, based on an AD strategy for gradient evaluation~\cite{sanchez2018}, the proposed approach is modular and based on a Python-wrapped interface between different solvers (i.e. CFD, FEM and interpolation). It is considered, in fact, that such approach is an ideal solution for a wider infrastructure in which more tools of various fidelity levels, provided with a standard interface, can be incorporated to perform both analysis and optimization at the different stages of the design process. It will also facilitate an easy access to high-fidelity multidisciplinary optimization tools for aircraft design to a potentially large user audience. PyBeam has also been developed as a model code to show how simple the integration of the chosen AD library (CoDiPack) would be on existing codes, avoiding manual implementations of adjoint algorithms which are usually complex at code level and time-consuming to perform, despite recent advantages in this direction~\cite{DAFoam2019}.
%%%%%%%%%
\subsection{Organization of the paper}
%%%%%%%%%%%
This work follows up a previous effort by Bombardieri \textit{et al.} \inred{cite book chapter}. In this work pyBeam module was presented and the primal aeroelastic solver was shown. Later on, the novel AD-based gradient evaluation strategy was introduced and the calculation of selected aerostructural cross sensitivities was validated. In the current work, pyBeam capabilities are extended with nonlinear rigid elements, the optimization framework is set up and applied to cases of industrial interest. The remainder of this paper is organized as follows: in Section~\ref{sec:theory} the theoretical background for the solution of the aerostructural problem and for sensitivities evaluation is fully detailed, in Section~\ref{sec:testcases} the aeroelastic test cases are introduced (i.e. aeroelastic models of the ONERA M6 wing and of the CRM), in Section~\ref{sec:results} AD-based aerosturctural sensitivities validation is presented and results of the optimization are shown and discussed. Section~\ref{sec:concl} contains the conclusions.

==> Chapters/IntroductionLONG.tex <==
 %------------------------------------------% 
% algorithm   Bezier                    %
%------------------------------------------%
\section{Introduction}
\label{sec:intro}
%------------------------------------------%
Multi Disciplinary optimization (MDO) applied to aircraft design has been attracting the interest of both research ind industry for the last fifty years. The appeal for tools that can automatically optimize aircraft configurations taking into account disciplines interaction at conceptual and preliminary design phases is growing. Thus is made more important by the advance of computer technologies, which is making always more affordable the use of higher-fidelity tools for performance predictions.
%
\par
% 
One of the first effort in this direction was done by Haftka~\cite{HAFTKA-1977} who proposed a method for the optimization of flexible wings subjected to stress, strain and drag constraints. In  such work, induced drag was calculated with a lifting line method and the structure with a Finite Element Method (FEM). A penalty method formulation was converting the constrained problem into an unconstrained one. 
Later on, Grossman \textit{et al.}~\cite{GROSSMAN_1986} applied an integrated aircraft design analysis and optimization on a sailplane, employing a lifting line model for aerodynamics and a FE beam model for structure. They explored two optimization approaches: in the first, aerodynamics and structure where optimized sequentially while in the second, an integrated procedure was used. They showed how the integrated approach is superior to the iterative approach, capitalizing on the interaction between disciplines and finding better results with respect to sub-optimal ones, given by sequential optimization. A physical interpretation of the different outcomes was also provided.
%
Following this last work, a higher-fidelity aerostructural model was later used for the optimization of the weight of a forward-swept subsonic aircraft wing subjected to range constraint~\cite{GROSSMAN_1989}. For the aerodynamics, a vortex lattice method was used and viscous drag estimation was computed using section lift coefficient and drag polar, based on provided data; various design variables were employed, based on geometry, structure and performance requirements. 
%
The advantage of coupled aerostructural optimization with respect to the sequential one was also recently confirmed by Martins \textit{et al.}\cite{Martins2004HighFidelityAD} employing an Euler flow model within the context of their aerostructural solver.
%
\par
%
In the last twenty years, studies have stated to employ higher-fidelity tools to investigate aerostructural couplings. One of the pioneering works in this direction is the one of Maute \textit{et al.}~\cite{maute_2001}. In this work a gradient-based optimization framework for aeroelastic problem was proposed. They used a three-field approach to model the the nonlinear coupled problem, employing a staggered procedure for the solution (also known as partitioned or segregated). Aerodynamics consisted in an Euler flow model, structure in a linear FEM model and the motion of the fluid grid was computed by means of a spring analogy method. It is stated that three-field formulations are on average 25\% slower than two-field ones but allow for bigger displacements in the structure, making it more general and reliable for a variety of cases. For the evaluation of sensitivity a direct approach was chosen, in which partial derivatives where analytically calculated and a staggered scheme was used to solve the system of equations. Direct approach is, anyway, only advantageous when then number of design variables is contained.
%
\par
%
Martins \textit{et al.}~\cite{martins2001ab} proposed a framework for the calculation of coupled aerostructural sensitivities for cases in which aeroelastic interactions are significant. The method is a two-field aeroselastic solver, employing high-fidelity models for both aerodynamics (Euler model) and structure (linear FEM with two element types). This work is considered, to the best of the authors' knowledge, one of the first efforts to employ an adjoint method for the evaluation of aerostructural sensitivities~\cite{Martins_Review_Der2013}. Such method allows a faster evaluation of sensitivities in case of a high number of design variables, making the computational time and cost to be almost independent on their number and, for such reason, the ideal to be applied for industrial cases. The proposed sensitivity evaluation framework is a lagged-coupled adjoint, in which the single discipline adjoint equations are lagged in a similar fashion of the primal solver solution strategy, and partial derivatives are evaluated analytically or by finite differences (FD). The proposed implementation was able to calculate aerostructural sensitivity of $C_D$ with respect to bump functions applied to deform the wing surface. Their accuracy was compared both to FD and complex step (CP)-based sensitivities.
%
\par
%
Following their previous effort~\cite{maute_2001}, Maute \textit{et al.}~\cite{maute2003911} proposed a different method for aeroelastic optimization. For the same aerostructural problem, gradient calculation was achieved by the authors by analytically deriving the adjoint-based sensitivity equations of the primal problem: a staggered solution algorithm was implemented, where partial derivatives could be calculated analytically or by automatic differentiation. They also pointed out the computational problems relative to store partial derivative matrices of large-scale problems for adjoint-based sensitivity calculations. 
%
\par
%
In a following effort\cite{Martins2004HighFidelityAD}, Martins \textit{et al.} use a similar optimization framework than the one presented at CEAS~\cite{martins2001ab} to optimize the design of a supersonic business jet. In this framework the flow was modeled with Euler equations while the structure consisted in a detailed linear FEM model. A comparison of adjoint-based sensitivities with FD and CP-based ones showed an average error of 2\%. The optimization was performed minimizing a combination of the aircraft $C_D$  and weight, constraining its $C_L$ and the Kreisselmeier-Steinhauser function to lump individual stresses of the structure. A total number of 97 design variables was used, divided into structural and aerodynamic surface ones, showing the almost independence of the gradient evaluation time from their number.
%
\par
%
The work of Barcelos \textit{et al.}~\cite{Barcelos20081813} presented an optimization methodology for fluid-structure interaction (FSI) problems based on turbulent flow models. The method employs the same three-field formulation strategy used in Maute \textit{et al.}~\cite{maute_2001,maute2003911} using a Reynolds Average Navier-Stokes (RANS) flow model based on the Spalart-Allmaras (SA) turbulence model, while the structure is modeled via a geometrically nonlinear FEM. This counts, to the best of the authors' knowledge, as the highest level of fidelity adopted so far for aerostructural optimization on aircraft wings. For the calculation of sensitivities the direct approach is followed, in which all partial derivatives contribution are evaluated analytically or via FD. Using the direct approach requires the evaluation of the total derivatives of the state variables of the coupled aeroelastic problem as many times as the number of design variables. Nevertheless it was considered an advantageous approach compared to the adjoint one in case of large-scale problems, for which the Jacobian of the flow problem is difficult to transpose and keep in memory to be used at need. This is one of the common drawbacks due to memory requirements when using adjoint-based sensitivity evaluation strategies, largely mentioned in literature~\cite{maute2003911,SanchezThesis} which, in the current effort, is conveniently solved with the use of the library CoDiPack~\cite{sagebaum2017high} for Algorithmic Differentiation (AD).
%
\par
%
Nikbay \textit{et al.}~\cite{Nickbay2009} opted for a different optimization strategy, more industry oriented, in which the software modeFRONTIER was used as a driver for a multi-objective genetic-based optimization algorithm, wrapping various commercial codes (FLUENT for Euler-based aerodynamics, ABAQUS for linear FEM-based structure and CATIA for parametric solid geometry handling) to perform a loosely coupled aeroelastic analysis. The framework was built to handle the interfaces between such codes and the approach was validated on two aeroelastic testcases: the AGARD 445.6 wing and the ARW-2 wing. The motivation of such effort is that corporate working cultures need to rely (partially or entirely) on assessed commercial codes and a winning strategy is to provide modular optimization frameworks for which each unit (conveniently interfaced) can be plugged and used. 
%
\par
%
Other efforts presented gradient-based aerostructural optimizations using adjoint methods. Brezillion \textit{et al.}~\cite{Brezillon2012} proposed an articulated high-fidelity optimization framework wrapping DLR's TAU code for CFD (performing RANS completed by a SA turbulence model) which includes a discrete-adjoint model with non-frozen turbulence and ANSYS for linear structural FEM. It is claimed, here, that relying only on high-fidelity models, besides being very costly, is unnecessary, and that multi-fidelity optimization strategies should be considered.
%
A similar approach has been pursued by Ghazlane \textit{et al.}~\cite{ghazlane2012}. In the presented aerostructural framework, CFD (Euler flow model) was handled by the ONERA elsA code~\cite{Cambier2002}, which used an iterative fixed-point scheme for the solution of the aerodynamic adjoint, while, for the structure, a linear structural FEM module was differentiated by hand.
%
\par
%
In effort~\cite{kenway2014} Kenway \textit{et al.} introduced a high-fidelity framework that can perform aeorelastic optimization with respect to thousands of multidisciplinary variable. This could be achieved with an improved parallel scalability of the method which features a Newton-Kyrlov approach for the solution of the coupled aerostructural and the relative adjoint systems. The aerostructural solver was based on SUmb~\cite{Weide2006} for  CFD, which is enabled with automatic differentiation (ADjoint), and TACS\cite{TACS2010} for structural FEM, which is also able to evaluate adjoint-based sensitivities. For this work Euler flow model was used together with a linear detailed FEM model of the structure. To solve the aerostructural adjoint equations a combination of analytic, forward, and reverse AD methods was adopted. The method was demonstrated on a CRM test case~\cite{Vassberg-2008} using a CFD mesh with over than $16 \times 10^6$ cells,  a computational structural mechanics (CSM) model with over $10^6$ degrees of freedom (DOF) and more than $8 \times 10^6$ state variables, using 512 processors. Driving motivation of the effort was that, nevertheless adjoint-based gradient evaluation techniques should be almost independent on the number of considered design variables, in all previous efforts in literature their number had been limited: this because the real scalability of the method can only be achieved with a careful parallelization of its implementation. Similarly, in another study~\cite{KenwayMultipoint2014} Kenway \textit{et al.} presented a multipoint high-fidelity aerostructutal optimization of a CRM aeroelastic model, minimizing the takeoff gross weight or the fuel burn. The CRM detailed CSM is built based on its aerodynamic mold line at 1 \textit{g} load factor. Flow model was based on Euler equation with a viscous drag estimate and structure was linear. They exploited a massively parallel supercomputer with more than 400 processors.
%
\par
%
Similar work was carried on by Kennedy \textit{et al.}\cite{Kennedy2014e} optimizing a Quasi-CRM wing model introducing also composite material for the structure. Gradient-based aerostructural optimization is carried out using medium-fidelity tools: a combination of a panel method enhanced with induced and viscous drag evaluation (Tripan) together with a linear structural model (TACS). For coupled aerostructural adjoint analytic derivatives are implemented in the framework. After an aerostructural optimization which aims at minimizing a linear combination of takeoff gross weight and fuel burn a final RANS-based (SUmb) aerodynamic shape optimization is performed over the winner configuration aiming at minimizing $C_D$. Add on to the study is done by the authors in a follwing effort~\cite{kennedyScitech2014}, in which RANS-based aerostructural optimizations are performed on the same aeroelastic model.
%
\par
%
Works of Kenway \textit{et al.}~\cite{KenwayScitech2014} and Brooks \textit{et al.}~\cite{Brooks2018} are dedicated to define, with an inverse design procedure and for aerostructural optimization purposes, undeflected versions with different Aspect Ratios (AR) of the CRM (uCRM). This because the CRM is born as aerodynamic benchmark only and its outer mold line represents the aerodynamic shape for 1 \textit{g} load factor. For the found configurations gradient-based aerostructural optimizations have been performed, employing RANS-based CFD and linear FEM model with a similar computational infrastructure as the one mentioned above by the same authors. 
%
\par
%
The study of Hoogervorst \textit{et al.}\cite{Hoogervorst2017WingAO} proposes an unconventional approach in the landscape of gradient-based aerostructural optimization. In such approach, based on the individual discipline feasible architecture, the various disciplines of the aerostructural problem are decoupled and convergence is ensured imposing additional equality constraints on the interdisciplinary state variables, which become additional design surrogate variables. This ensures to keep low the computational cost of the problem, especially in cases of strong nonlinearities, but only when the increase in design variables is kept low. In this study, flow is modeled with the Euler equation using the open-source code SU2~\cite{SU2_AIAAJ2016} while the analysis tool FEMWET is used to solve the linear structural equations. A combination of continuous adjoint approach and FD is used for gradient evaluation. The method is applied to reduce the fuel weight of an Airbus A320 aircraft for the specified range. Design variables are defined as the displacements of a Free-Form Deformation (FFD) box control points and selected structural model panels thicknesses, together with the additional surrogate variables requested by the approach.
%
\par
%
Another conspicuous branch of works in the field of aerostructural optimization relies on the use of low-medium fidelity aerodynamic models for the aeroelastic system. This is justified by the fact that using only high fidelity models in MDO makes the problem computationally too expensive to be employed in early design stages, where multiple designs are being considered at the same time. Besides the already mentioned work of of Kennedy \textit{et al.}~\cite{Kennedy2014e}, it is worth reporting efforts of Chauhan \textit{et al.}~\cite{Chauhan2018LowFidelityAO} and Jasa \textit{et al.}~\cite{Jasa2018OpensourceCA}, employing OpenAeroStruct: an open-source aerostructural optimization framework which couples a Vortex Lattice Method (VLM) to a 1D FEM to model lifting surfaces and uses coupled adjoint for gradient-based optimization, performed by means of NASA's OpenMDAO~\cite{OpenMDAO2012}. The framework presented by Elham \textit{et al.}~\cite{Elham2015} is a method for aerostructural optimization based on a VLM for aerodynamics and a beam model for structural FEM. With the enhancement of a viscous compressible airfoil drag prediction code, it is claimed to have a level of accuracy comparable to higher fidelity CFD-based tools. Sensitivities are evaluated with a combination of coupled adjoint method, automatic differentiation and chain rule differentiation.
%
\par
%
The studies mentioned above, mostly in chronological order, represent a part of the attempt of the aerospace community to perform coupled aerostructural optimization applied to aircraft wings, with particular emphasis on frameworks relying on high-fidelity CFD and CSM models. Main contribution of this work is to introduce an open-source, high-fidelity framework for aeorstructural design and optimization of wings, including aerodynamic and structural nonlinearities. The proposed gradient-based optimizator  relies on an innovative and, to the best of the author's knowledge, never used strategy, based on coupled AD for gradient evaluation, which includes nonlinearities both in the CFD and CSM problems. The framework, to be part of the open-source SU2 suite~\cite{Palacios2015, Pini2017, Gori2017, Molina2017, Zhou2017, albring2016}, relies on SU2 for high-fidelity CFD (Euler, RANS) and on a geometrically nonlinear beam FEM solver, namely pyBeam. Differently than previous efforts, in which FSI optimization problems were tackled by SU2 at native level, based on an AD strategy for gradient evaluation~\cite{sanchez2018}, the proposed approach is modular and based on a python wrapped interface between different solvers (i.e. CFD, FEM and interpolation). It is considered, in fact, that such approach is an ideal solution for a wider infrastructure in which more tools of various fidelity levels, provided with a standard interface, can be incorporated to perform both analysis and optimization at the different stages of the design process. It will also facilitate an easy access to high-fidelity multidisciplinary optimization tools for aircraft design to a potentially large user audience. PyBeam has also been developed as a model code to show how simple the integration of the chosen AD library (CoDiPack) would be on existing codes, avoiding manual implementations of adjoint algorithms which are usually complex at code level and time-consuming to perform, despite recent advantages in this direction~\cite{DAFoam2019}.
%
\par
%
This work follows up a previous effort by Bombardieri \textit{et al.} \inred{cite book chapter}. In this work pyBeam module was presented and the primal aeroelastic solver was shown. Later on, the novel AD-based gradient evaluation strategy was introduced and the calculation of selected aerostructural cross sensitivities was validated. In the current work, pyBeam capabilities are extended with nonlinear rigid elements, the optimization framework is set up and applied to cases of industrial interest. The remainder of this paper is organized as follows: in Section~\ref{sec:theory} the theoretical background for the solution of the aerostructural problem and for sensitivities evaluation is fully detailed, in Section~\ref{sec:testcases} the aeroelastic test cases are introduced (i.e. aeroelastic models of the ONERA M6 wing and of the CRM), in Section~\ref{sec:results} AD-based aerosturctural sensitivities validation is presented and results of the optimization are shown and discussed. Section~\ref{sec:concl} contains the conclusions.


==> bibliography/FP_adjoint.tex <==
\newpage
\begin{subequations} \label{e:adjoint}
\begin{equation} \label{e:ad_w} 
\frac{\partial J}{\partial \mathbf{w}} + 
\mathbf{\bar{w}}^T_n \left. \frac{\partial  \mathrm{\mathbf{F}} }{\partial \mathbf{w}} \right|_{\mathbf{w^*}, \mathbf{z^*}} + 
\mathbf{\bar{f}_{f}}^T \;  \left. \frac{\partial  \mathrm{\mathbf{F_f}} }{\partial \mathbf{w}} \right|_{\mathbf{w^*}, \mathbf{z^*}} = \mathbf{\bar{w}}^T_{n+1}
\end{equation}
\\
\begin{equation} \label{e:ad_z} 
\frac{\partial J}{\partial \mathbf{z}} + 
\mathbf{\bar{w}}^T \;  \left. \frac{\partial  \mathrm{\mathbf{F}} }{\partial \mathbf{z}} \right|_{\mathbf{w^*}, \mathbf{z^*}} + \mathbf{\bar{f}_{f}}^T \;  \left. \frac{\partial  \mathrm{\mathbf{F_f}} }{\partial \mathbf{z}} \right|_{\mathbf{w^*}, \mathbf{z^*}} +  \mathbf{\bar{z}}^T = 0
\end{equation}
\\
\begin{equation} \label{e:ad_utot} 
\frac{\partial J}{\partial \mathbf{u_{tot}}} + 
\mathbf{\bar{z}}^T \;  \left. \frac{\partial  \mathrm{\mathbf{M}} }{\partial \mathbf{u_{tot}}} \right|_{\mathbf{u_{tot}^*}} + \mathbf{\bar{u}_{tot}}^T = 0
\end{equation}
\\
\begin{equation} \label{e:ad_uf} 
\frac{\partial J}{\partial \mathbf{u_f}} - \mathbf{\bar{u_{f}}}^T - \mathbf{\bar{u}_{tot}}^T = 0
\end{equation}
\\
\begin{equation} \label{e:ad_us} 
\frac{\partial J}{\partial \mathbf{u_s}} + \mathbf{\bar{u}_s}_n^T  \left. \frac{\partial  \mathrm{\mathbf{S}} }{\partial \mathbf{u_s}} \right|_{\mathbf{u_s^*}, \mathbf{f_s^*}} + 
 \mathbf{\bar{u_{f}}}^T \;  \mathbf{H}_{MLS} = \mathbf{\bar{u}_s}_{n+1}^T
\end{equation}
\\
\begin{equation} \label{e:ad_fs} 
 \frac{\partial J}{\partial \mathbf{f_s}} + \mathbf{\bar{u}_s}^T \left. \frac{\partial  \mathrm{\mathbf{S}} }{\partial \mathbf{f_s}} \right|_{\mathbf{u_s^*}, \mathbf{f_s^*}} - 
 \mathbf{\bar{f}_{s}}^T  = 0
\end{equation}
\\
\begin{equation} \label{e:ad_ff} 
 \frac{\partial J}{\partial \mathbf{f_f}} -\mathbf{\bar{f}_{f}}^T + \mathbf{\bar{f}_{s}}^T \;  \mathbf{H}_{MLS}^T = 0
\end{equation}
\\
\begin{equation}\label{eq:gradient_dvs}  
\frac{\partial J}{\partial  {\mathbf{u_{F_{\alpha}}}}} - \mathbf{\bar{u}_{tot}}^T = \frac{\mathrm{d} J}{\mathrm{d} {\mathbf{u_{F_{\alpha}}}}} 
\end{equation}
\end{subequations}
